Quantifying Human Priors over Social and Navigation Networks

Human knowledge is largely implicit and relational -- do we have a friend in common? can I walk from here to there? In this work, we leverage the combinatorial structure of graphs to quantify human priors over such relational data. Our experiments focus on two domains that have been continuously relevant over evolutionary timescales: social interaction and spatial navigation. We find that some features of the inferred priors are remarkably consistent, such as the tendency for sparsity as a function of graph size. Other features are domain-specific, such as the propensity for triadic closure in social interactions. More broadly, our work demonstrates how nonclassical statistical analysis of indirect behavioral experiments can be used to efficiently model latent biases in the data.

==> 007ResultsPart1ScaledCumulants.tex <==
\subsection{Substructures with Noticeable Trends in the Priors}
\label{ssec:resultsedgewedgetriangle}
We now present the results for: edge density {\muEdgeText} (fig.~\ref{fig:sparsepriors}), scaled cherry cumulant {\scaledCumWedgeText} (fig.~\ref{fig:egalitarian}), and scaled triangle cumulant {\scaledCumTriangleText} (fig.~\ref{fig:socialtriangles}) for each of the four cover stories as a function of the number of nodes in the prior.\footnote{Despite number of nodes clearly being a discrete variable, we plot the results as curves to aid in the visualization of the trends.}
Intuitively, these statistics quantify \mbox{well-known} tendencies of real networks: sparsity, degree heterogeneity, and clustering, respectively.
It is then perhaps not a coincidence that those were indeed the substructures that displayed the most discernible trends across the priors.
%








% \begin{figure*}[ht] 
% % \vskip 0.2in
% 	\begin{center}
%   \centering
% % trim={<left> <lower> <right> <upper>}
% % \includegraphics[trim={0.5cm 0 0 0},clip,width=\columnwidth]
%           \begin{subfigure}[t]{0.667\columnwidth}
%   \centering
%       \includegraphics[trim={0.09cm 0.1cm 0 0},clip,width=1\columnwidth]{Figures/2023SparsePlot.pdf}
%        % \vspace{-0.05in}
%     \caption{\textbf{Larger graphs are more sparse}}
%     \label{fig:sparsepriors}
%     \end{subfigure}
%     % \hfill
%      ~
%       \begin{subfigure}[t]{0.667\columnwidth}
%   \centering
%     \includegraphics[trim={0.09cm 0.1cm 0 0},clip,width=1\columnwidth]{Figures/2023WedgePlot.pdf}
%      % \vspace{-0.05in}
%     \caption{\textbf{Smaller graphs have fewer hubs}}
%     \label{fig:egalitarian}
%     \end{subfigure}
%      % \hfill
%      ~
%   \hspace{1pt}
%     \begin{subfigure}[t]{0.667\columnwidth}
%    \includegraphics[trim={0.09cm 0.1cm 0 0},clip,width=1\columnwidth]{Figures/2023TrianglePlot.pdf}
%     % \vspace{-0.05in}
%    \caption{\textbf{Social graphs have more triangles}}
%      \label{fig:socialtriangles}
%    \end{subfigure}
%     % \vspace{-0.05in}
%   \caption{\tocheck{\textbf{Values in the participants' priors of three statistics that quantify \mbox{well-known} tendencies of real networks.}\\
% The markers in the solid curves correspond to the measured values in participants' priors for: \textbf{(a)} edge density (quantifies preference in density of connections), \textbf{(b)} scaled cherry cumulant (quantifies preference for degree heterogeneity), and \textbf{(c)} scaled triangle cumulant (quantifies preference for clustering). % $ER_{n,\mu_{\Edge}^{ }}$ % triadic closure
% In \textbf{(b)} a negative value indicates that the prior has edges distributed more uniformly than would be expected by chance (i.e., in an \mbox{$ER_{n,\rho}$} distribution with same number of nodes $n$ and edge density \mbox{$\rho=\mu_{\Edge}^{ }$}). 
% Likewise, in \textbf{(c)} a negative value indicates that the prior has fewer triangles than would be expected by chance. 
%   Each prior was inferred using the aggregated data of a single cover story for a fixed number of nodes (Section~\ref{sec:errorbarplots} and Appendix~\ref{app:fittingprocedure}). 
%   The region encompassed by the shading corresponds to one standard deviation of the average value that would have been obtained if participants behaved exactly accordingly to the model and using the corresponding inferred prior (Section~\ref{sec:errorbarplots}).
%   Note that the result of this procedure does not need to be centered around the empirical values (i.e., the solid curves).
%   }  
%  }
%     \label{fig:threesubgraphs}
% 	 \end{center}	
% \vskip -0.2in	
% \end{figure*}
\vspace{-8pt}
\paragraph{Priors favor sparsity.} 
As shown in figure~\ref{fig:sparsepriors}, 
we find that the edge density systematically decreases as the number of nodes increases.  
% This result is remarkably similar between the different cover stories. 
The number of connections \textit{per node}, however, appears to be a slowly increasing function of the number of nodes in the graph. 
These results are remarkably similar for all the different cover stories. 
% In particular, the number of connections \textit{per node} appears to be a slowly increasing function of the number of nodes in the graph.
\input{007ResultsFig1EdgeDensity.tex}
%%%%%%%%%%
%%%%%%%%%%
\paragraph{Priors favor similar degrees in small graphs.} 
As shown in figure~\ref{fig:egalitarian},
we find that the preference for degree heterogeneity (i.e., a few ``hub'' nodes with large degree) 
increases as the number of nodes increases. 
% Across all cover stories the scaled cumulant for the cherry subgraph \mbox{$\kappa_{\Wedge}/\mu^2_{\Edge}$} changes from negative (for graphs with $4$ or $5$ nodes) to positive (for graphs with $6$ or more nodes).  
Across all cover stories the scaled cumulant for the cherry subgraph 
{\scaledCumWedgeText}
changes from negative (for graphs with $4$ or $5$ nodes) to positive (for graphs with $6$ or more nodes).  
This suggests that human priors favor an exceptionally uniform distribution of node degrees for small graphs, switching to a preference for heterogeneous node degrees for larger graphs.
\input{007ResultsFig2Cherries.tex}
%%%%%%%%%%
%%%%%%%%%%
\paragraph{Priors over social interactions favor triangles.} 
While the trends of edge density and degree heterogeneity are similar across our cover stories, 
as shown in figure~\ref{fig:socialtriangles},
the scaled triangle cumulant {\scaledCumTriangleText} reveals that the social domain has a notably higher preference for clustering. 
% the scaled triangle cumulant {\scaledCumTriangleTextNotSmash} reveals that the social domain has a notably higher preference for clustering. 
Indeed, \citet{tompson2019individual} found experimental evidence that humans learn community structure differently when the network is social vs.~\mbox{non-social}, 
and the prevalence of triadic closure in social networks (i.e., one's friends tend to be friends with each other) is a \mbox{well-established} phenomenon \cite{yang2016social}.
\input{007ResultsFig3Triangles}
% (e.g., there are over \mbox{$12\cdot10^6$} different graphs with $10$ nodes),

==> 007ResultsPart1bEdgeBimodality.tex <==
% (e.g., there are over \mbox{$12\cdot10^6$} different graphs with $10$ nodes),
%%%%%%%%%%
%%%%%%%%%%
\paragraph{Extending to priors over more nodes.} 
Perhaps frustratingly, the above results end at graphs with eight nodes.  
While we also collected data for graphs with a larger number of nodes (i.e.,  $10$, $12$, and $15$, see Appendix~\ref{app:experimentaldesign}), 
obtaining meaningful results for these graphs presents two major challenges.
% obtaining meaningful results for graphs with $\gtrsim8$ nodes presents two major challenges.
As the number of unique graphs increases\footnote{E.g., there are over \mbox{$12\cdot10^6$} different graphs with $10$ nodes.} 
fitting the model exactly becomes computationally infeasible (see Appendix~\ref{app:scalability}).  
Additionally, in practice, the attention and engagement of the participants appears to notably decrease when presented with this amount of questions and constraints.

To overcome at least the computational impasse of larger graphs, 
we consider restricting attention to \textit{only} the edge density.  
Specifically, we consider maximum entropy distributions over the number of edges. 
This reduces the domain of the priors to \mbox{${n\choose2} +1$} (i.e., all graphs with the same number of edges are considered to be the same by the model), and we use the observed moments of the edge density as constraints for these maximum entropy distributions.
Using this approach we are able to analyze the structure of the priors over the number of connections only (i.e., neglecting the details of the graphical structure).
The results for priors with the first six moments constrained are shown in Figure~\ref{fig:edgedensityallnodes}.

\input{007ResultsFig4EdgeBimodality.tex}

% \vspace{-30pt}
\paragraph{Appearance of bimodality in priors over connections.}
Surprisingly, for graphs with \mbox{$n\gtrsim8$} nodes, 
these priors become notably bimodal.
Sparse graphs are easier to remember as they admit a natural compression. 
This compression may equally well be applied to their complements (i.e., the \mbox{nearly-complete} graphs) 
by remembering the ``\mbox{non-edges}''.  
Below \mbox{$n\lesssim7$} nodes, the sparse peak and its dense complement overlap considerably.  
As the number of nodes increases, the dense peak is increasingly \mbox{well-separated} from its sparse complement.  

While it is tempting to draw conclusions about this ``regime change'', 
it is worth remembering that human engagement for these larger graphs is still questionable; 
it is possible that these results are a product of their desire to complete the task.
Indeed, in our \mbox{post-questionnaires}, some participants suggested that cognitive fatigue may have played a role. 
And with $105$ pairwise relationships between $15$ nodes, 
it would not be unreasonable to reduce the computational cost by choosing a ``simple'' solution (such as nearly zero connections or nearly all connections).
% \vspace{10pt}

==> 007ResultsPart2ComparingCoverStories.tex <==
\subsection{Generalization Between and Within Domains}
\label{ssec:generalizationresults}
We now consider how the priors generalize within and between domains 
as a function of model complexity (parameterized by $r$ in eq.~\ref{eq:LowDimensionalPrior}, see also section~\ref{sec:modelselection}).
To this end, for each number of nodes, we randomly partitioned the data from each cover story into a training set ($80\%$) and a test set ($20\%$).  
We fit a model to each set of training data 
and measured the \mbox{log-likelihood} (per round) of each set of test data.  
We then normalized these quantities by the \mbox{log-likelihood} (per round) of the test data given a ``\mbox{non-specialized} model'' (i.e., one that was fitted to the aggregated training data for all four cover stories).  
Thus, a value of $1.00$ corresponds to the specialized model explaining the data equally as well as the \mbox{non-specialized} model, while a value greater than one indicates that the specialized model explains the data better than the \mbox{non-specialized} model (and conversely for a value less than one). 
The cells in figure~\ref{fig:comparisonwithfitorder} show the average result of $64$ repetitions of this procedure (for that particular number of nodes, model complexity $r$, and combination of cover stories used for testing/training). 

% consistent across all number of nodes,
\input{007ResultsFig5CoverStoriesComp.tex}
\paragraph{Larger subgraphs reveal differences between domains.}
As a general trend, we find that more complex models recover priors that are better able to differentiate between domains and (to a lesser degree) specific cover stories.  This is reflected in the suggestively ``block-diagonal'' appearance of \mbox{$r=6$} in fig.~\ref{fig:comparisonwithfitorder}.  
The ``row/horizontal'' appearance of \mbox{$r=1$} suggests that the quality of fit for less complex models is determined primarily by the particular data used for testing.  
% Indeed, as one would expect more specific models to be able to better distinguish different domains.
%
% One aspect of our experiments that warrants mentioning is the duality between the two spatial navigation cover stories.
% \new{An aspect of our experiments that warrants mentioning is the duality between the two spatial navigation cover stories.}  

One aspect worth mentioning is the duality between our two spatial navigation cover stories. 
While both were suggestively planar, their connectivity was of two different forms. 
The trails are rather analogous to \mbox{vectors} (a ``large'' trail implies a large separation between the two sites), while the boundaries between neighborhoods are analogous to \mbox{one-forms} (a ``large'' boundary between neighborhoods implies that they are nearby).  
Although one might expect that this dual representation would result in different priors, the similarity between the priors for the two navigation cover stories is about the same as the similarity between those for the two social cover stories.  
% led to priors that are as similar to each other as the priors for the two social cover stories are to each other. 
% \begin{figure}[ht] 
% \vskip -0.1in
% \begin{center}
% 	% \includegraphics[width=0.5\textwidth]{expressivesquares.pdf}
%  	\centerline{\includegraphics[trim={1cm 0 0 0},clip,width=1.02\columnwidth]{Figures/ExpressiveSquares.pdf}}
% % \end{center}
% % \caption{\textbf{\mbox{Higher-order} substructures reveal differences between domains.}  \\
% % \textbf{Larger substructures reveal differences between domains.}  \\
% \caption{\textbf{\new{Larger motifs reveal differences between domains.}} 
% For each of the 4$\times$4 squares, we fit our model to the data indicated by the (sub)row, and evaluated its performance on the data indicated by the (sub)column.  
% % For each square, the number is \mbox{color-coded} to aid in visualization, 
% % with d
% % \tocheck{The complexity of the fit (i.e., the $r$ in Eq.~\eqref{eq:LowDimensionalPrior})
% % }
% \tocheck{From left to right, the structural complexity $r$ of the inferred prior (Eq.~\eqref{eq:LowDimensionalPrior}) ranges from $1$ (edges are placed i.i.d.~with probability $\rho$, i.e., an $\textrm{ER}_{n,\rho}$ model) to $6$ (the prior considers the density of all subgraphs with $\leq6$ edges).}
% Darker colors indicate a better fit of the specialized model.
% % , and lighter colors indicate a worse fit.  
% % of the specialized model.
% % (see main text for detailed description). 
% \new{The specific numbers are less important than the overall trend:} 
% \new{for simpler models, specialization between domains is not particularly apparent, while for more complex models there is sufficient resolution to distill a \mbox{2$\times$2} block structure, indicating that priors for one cover story generalize better to cover stories in the same domain.} 
% % The specific numbers are not as important as the overall trend from left to right: 
% % \new{for \mbox{lower-order} (simpler) models, specialization between domains is not particularly apparent, while for \mbox{higher-order} (more complex) models there is sufficient resolution to distill a \mbox{2$\times$2} block structure, indicating that priors for one cover story generalize better to cover stories in the same domain.} 
% % from one cover story better generalize to cover stories in the same domain.
% }
% \label{fig:comparisonwithfitorder}
% \end{center}
% \vskip -0.4in
% \end{figure}
%
% \centerline{ \includegraphics[trim={0.27cm 0.3cm 0 0},clip,width=0.85\columnwidth]{Figures/2023SparsePlot.pdf}} % trim={<left> <lower> <right> <upper>}
%
% \input{007ResultsFig5CoverStoriesComp.tex}

==> TextForLabelofFigures.tex <==

\textbf{\classcolor{Class}} 

\textbf{\workcolor{Work}}

\textbf{\trailcolor{Park}}

\textbf{\citycolor{City}}


\classcolor{Class} 

\workcolor{Work}

\trailcolor{Park}

\citycolor{City}

\textbf{\textsc{\classcolor{Class}}} 

\textbf{\textsc{\workcolor{Work}}}

\textbf{\textsc{\trailcolor{Park}}}

\textbf{\textsc{\citycolor{City}}}


\classcolor{\textsc{Class}}

\workcolor{\textsc{Work}}

\trailcolor{\textsc{Park}}

\citycolor{\textsc{City}}

Edge density

Number of nodes

Scaled cherry cumulant

Scaled triangle cumulant 

Probability density

\textbf{Edge density}

\textbf{Number of nodes}

\textbf{Scaled cherry cumulant}

\textbf{Scaled triangle cumulant} 

\textbf{Probability density}



\newpage
\textbf{\classcolor{class}} 

\textbf{\workcolor{work}}

\textbf{\trailcolor{park}}

\textbf{\citycolor{city}}


\classcolor{class} 

\workcolor{work}

\trailcolor{park}

\citycolor{city}

\textbf{\textsc{\classcolor{class}}} 

\textbf{\textsc{\workcolor{work}}}

\textbf{\textsc{\trailcolor{park}}}

\textbf{\textsc{\citycolor{city}}}


\classcolor{\textsc{class}}

\workcolor{\textsc{work}}

\trailcolor{\textsc{park}}

\citycolor{\textsc{city}}

edge density

number of nodes

scaled cherry cumulant

scaled triangle cumulant 

probability density

\textbf{edge density}

\textbf{number of nodes}

\textbf{scaled cherry cumulant}

\textbf{scaled triangle cumulant} 

\textbf{probability density}

==> figuresquareoldcaption.tex <==
\begin{figure*}[hbt!]
\begin{center}
  \centerline{\includegraphics[trim={0 0 0 0},clip,width=2.00\columnwidth]{Figures/NewExpressiveSquaresNew.pdf}}
\vspace{-0.1in}
\caption{\textbf{Increasing the expressivity of the model for the priors reveals \mbox{domain-specific} traits.}\\ 
The \mbox{$4$-by-$6$} layout divides the results by the number of nodes \smash{\mbox{$4\leq n\leq7$}} (rows) and the model complexity \smash{\mbox{$1\leq r\leq6$}} (columns) of the priors. 
Each of these $24$ options for $n$ and $r$ contains results summarized by a \mbox{$4$-by-$4$} square of numbers. 
For each of these \mbox{$4$-by-$4$} square, we fit $4$ ``specialized'' models 
(using the training data of each cover story separately), 
as well as one ``\mbox{non-specialized}'' model 
(using the combined training data of all $4$ cover stories).  
As seen in the amplified \mbox{$4$-by-$4$} square on the right, 
the $4$ columns denote the cover story of the specialized training data, 
and the $4$ rows denote the cover story of the test data used to evaluate these models. 
The $16$ numbers in each \mbox{$4$-by-$4$} square are defined in section~\ref{ssec:generalizationresults} and rounded to the nearest $0.01$.  
They can be approximately thought of as an average \mbox{log-odds-ratio}; 
a value of \mbox{$1\pm\varepsilon$} corresponds to the case when the specialized model 
assigns a probability to an actual response of a participant 
that is about \mbox{$1\pm\varepsilon$} times the probability assigned by the \mbox{non-specialized} model. 
The coloring of the squares is purely for visualization; 
we scale the same range of colors to that square's maximum and minimum values. 
While the less expressive models (to the left) are in fact much more similar than the colors suggest, 
the more expressive models recover priors that are better able to differentiate between domains and (to a lesser degree) specific cover stories. 
% This is reflected in the suggestively ``\mbox{block-diagonal}'' appearance of the columns for \smash{\mbox{$r\gtrsim3$}}. 
% Conversely, the ``\mbox{horizontal-row}'' appearance of the columns for \smash{\mbox{$r\lesssim2$}} suggests that the quality of fit for less complex models is determined primarily by the particular data used for testing. 
}
\label{fig:comparisonwithfitorder}
\end{center}
\end{figure*}

==> test.tex <==
\subsubsection{test}

lalala
